Geometric Methods for Robust Data Analysis in High Dimension

Machine learning and data analysis now finds both scientific and industrial application in biology, chemistry, geology, medicine, and physics. These applications rely on large quantities of data gathered from automated sensors and user input. Furthermore, the dimensionality of many datasets is extreme: more details are being gathered about single user interactions or sensor readings. All of these applications encounter problems with a common theme: use observed data to make inferences about the world. Our work obtains the first provably efficient algorithms for Independent Component Analysis (ICA) in the presence of heavy-tailed data. The main tool in this result is the centroid body (a well-known topic in convex geometry), along with optimization and random walks for sampling from a convex body. This is the first algorithmic use of the centroid body and it is of independent theoretical interest, since it effectively replaces the estimation of covariance from samples, and is more generally accessible. This reduction relies on a non-linear transformation of samples from such an intersection of halfspaces (i.e. a simplex) to samples which are approximately from a linearly transformed product distribution. Through this transformation of samples, which can be done efficiently, one can then use an ICA algorithm to recover the vertices of the intersection of halfspaces. Finally, we again use ICA as an algorithmic primitive to construct an efficient solution to the widely-studied problem of learning the parameters of a Gaussian mixture model. Our algorithm again transforms samples from a Gaussian mixture model into samples which fit into the ICA model and, when processed by an ICA algorithm, result in recovery of the mixture parameters. Our algorithm is effective even when the number of Gaussians in the mixture grows polynomially with the ambient dimension

==> ch4.end.tex <==
\chapter{Contributions and Future Work}
\label{end.ch}

We have successfully shown in Chapter~\ref{implem.ch} how the problems
of having a cow can be solved. A lot of work can still be done in this
field so that better and bigger cows can be had. This is a matter
which can be pursued by those weeny grad students who have just
started their Ph.D. 

In reality, this document has been prepared by Manas Mandal and Al
Fencl to assist people in using the {\tt osudissert96} class for
\LaTeX\ to generate masters theses and doctoral dissertations at the Ohio
State University. The relevant files are available from the Department
of Computer and Information Science or Electrical Engineering.  Also, ask
around your department; the files may have already migrated to a computer
in your home department.

Keep in mind that this document {\em is not intended to teach you
\LaTeX\ } nor should it be used as such.  Lamport's book
\cite{lamport:latex} is a very good introduction to the wonderful
world of \LaTeX\ and it would be well worth your while to purchase
that book!

It is our sincere hope that the use of this document and the related
style files will help you in producing your thesis and/or
dissertation. We wish you ``Good Luck''!


==> direct_membership.tex <==
\section{Membership oracle for the centroid body}\label{sec:direct_membership}
%We will see now how to implement an $\eps$-weak membership oracle for $\Gamma X$ directly.
We will now describe and theoretically justify a new and practically efficient $\eps$-weak membership oracle for $\Gamma X$, which is a black-box that can answer approximate membership queries in $\Gamma X$.
\iflong
More precisely:
\begin{definition}%[\cite{GLS}]\label{def:eps-weak-oracle}
The \emph{$\epsilon$-weak membership problem} for $K\subseteq \RR^n$ is the following:
Given a point $y \in \QQ^n$ and a rational number $\eps > 0$, 
% \lnote{membership?}
%% oracle}
%%for a set $K\subseteq \RR^n$ is an oracle that 
either (i) assert that $y \in K_\eps$, or (ii) assert that $y \not \in K_{-\eps}$.
%% \begin{enumerate}
%% \item asserts that $y \in S(K,\eps)$, or
%% \item asserts that $y \not \in S(K,-\eps)$.
%% \end{enumerate}
An \emph{$\epsilon$-weak membership oracle} for $K$ is an oracle that solves the weak membership problem for $K$.
For $\delta \in [0,1]$, an \emph{$(\eps, \delta)$-weak membership oracle} for $K$ acts as 
follows: Given a point $y \in \QQ^n$, with probability at least $1-\delta$ it solves the  
$\eps$-weak membership problem for $y, K$, and otherwise its output can be arbitrary.  
\end{definition}
\iflong
We start with an informal description of the algorithm and its correctness.
\else
We give an informal description of the algorithm and its correctness.
\fi
%The oracle is much simpler and practical than the one described in \cite{anon_htica}. In particular, it does not need to deal with polarity algorithmically, as the polar is computed explicitly as part of the analysis
\else
\section{Membership oracle for the centroid body, without polarity}\label{sec:direct_membership}
We will see now how to implement an $\eps$-weak membership oracle for $\Gamma X$ directly, without using polarity. We start with an informal description of the algorithm and its correctness.
\fi

The algorithm implementing the oracle (Subroutine \ref{sub:centroid-oracle}) is the following: 
Let $q \in \RR^\dim$ be a query point. 
Let $X_1, \dotsc, X_N$ be a sample of random vector $X$.
Given the sample, let $Y$ be uniformly distributed in $\{X_1, \dotsc, X_N\}$. 
Output YES if $q \in \Gamma Y$, else output NO.

Idea of the correctness of the algorithm: If $q$ is not in $(\Gamma X)_\eps$, then there is a hyperplane separating $q$ from $(\Gamma X)_\eps$. 
Let $\{x \suchthat a^T x = b \}$ be the hyperplane, satisfying $\norm{a} = 1$, $a^T q > b$ and $a^T x \leq b$ for every $x \in (\Gamma X)_\eps$.
Thus, we have $h_{(\Gamma X)_\eps}(a) \leq b$ and $h_{\Gamma X}(a) \leq b - \eps$.
We have $h_{\Gamma Y}(a) = \e(\abs{a^T Y}) = (1/N) \sum_{i=1}^N \abs{a^T X_i}$. 
\iflong
By Lemma \ref{lem:1-plus-eps-chebyshev}, 
\else
By \cite[Lemma 14]{anon_htica},
\fi
$(1/N) \sum_{i=1}^N \abs{a^T X_i}$ is within $\eps$ of $\e \abs{a^T X} = h_{\Gamma X}(a) \leq b - \eps$ when $N$ is large enough with probability at least $1-\delta$ over the sample $X_1, \dotsc, X_N$. 
In particular, $h_{\Gamma Y}(a) \leq b$, which implies $q \notin \Gamma Y$ and the algorithm outputs NO, with probability at least $1-\delta$. 

If $q$ is in $(\Gamma X)_{-\eps}$, let $y = q + \eps \hat q \in \Gamma X$.  
\iflong
We will prove the following claim: 
\fi

\iflong
Informal claim (Lemma \ref{lem:centroid_approximation}): 
\else
Claim: 
\fi
For $p \in \Gamma X$, for large enough $N$ and with probability at least $1-\delta$ there is $z \in \Gamma Y$ so that $\norm{z - p} \leq \eps/10$. 

This claim applied to $p=y$ to get $z$, convexity of $\Gamma Y$ and the fact that $\Gamma Y$ contains $B \simeq \sigma_{\min}(A) B_2^\dim$ 
\iflong
(Lemma \ref{lem:innerball}) 
\fi
imply that $q \in \conv (B \cup \{ z \}) \subseteq \Gamma Y$ and the algorithm  outputs YES.

\iflong
We will prove the claim now. Let $p \in \Gamma X$. 
By the dual characterization of the centroid body (Proposition \ref{prop:dualcharacterization}), 
there exists a function $\lambda:\RR^\dim \to \RR$ such that $p = \e (\lambda(X) X)$ with $-1 \leq \lambda \leq 1$.
%there exists an $\dim$-dimensional probability measure $\nu$ such that $p = \int x \ud \nu(x)$ with $\ud \nu/ \ud \measure_X \leq 2$. 
Let 
%\[
%z = \frac{1}{N} \sum_{i=1}^N X_i \frac{\ud \nu}{\ud \measure_X}(X_i).
%\]
\(
z = \frac{1}{N} \sum_{i=1}^N \lambda(X_i) X_i.
\)
%We have $\e_{X_i} (X_i \frac{\ud \nu}{\ud \measure_X}(X_i)) = p$ and $\e_{X_i} ( \abs{X_i \frac{\ud \nu}{\ud \measure_X}(X_i)}^{1+\gamma}) \leq 2^{1+\gamma}\e_{X_i} ( \abs{X_i}^{1+\gamma}) \leq 2^{1+\gamma} M$. 
We have $\e_{X_i} (\lambda(X_i) X_i) = p$ and $\e_{X_i} ( \abs{\lambda(X_i) X_i}^{1+\gamma} ) \leq \e_{X_i} ( \abs{X_i}^{1+\gamma} ) \leq M$.
\iflong
By Lemma \ref{lem:1-plus-eps-chebyshev}
\else
By \cite[Lemma 14]{anon_htica}
\fi
and a union bound over every coordinate we get $\pr( \norm{p - z} \geq \eps) \leq \delta$ for $N$ large enough. 
\fi 

\iflong
\subsection{Formal Argument}
\else
We conclude with the main formal claims of the argument and a precise description of the oracle below:
\fi
%\ifcolt
\iflong
\begin{lemma}[\cite{anon_htica}]\label{lem:centroid-scaling}
Let $S = (S_1, \dots, S_n) \in \RR^n$ be an absolutely symmetrically distributed random vector such that
% $\e S = 0$\lnote{superfluous?}
$\e (\abs{S_i}) = 1$ for all $i$.
Then $B_{1}^{\dim} \subseteq \Gamma S \subseteq [-1,1]^\dim$.
%\lnote{we may want to state the stronger version with $B_1^n$}
%That is, the centroid body of $S$ contains the standard $\ell_1$-ball and is contained in the unit hypercube.
Moreover, $\dim^{-1/2} B_2^\dim \subseteq (\Gamma S)^\polar \subseteq \sqrt{\dim}B_2^\dim$.
\end{lemma}

\begin{lemma}[\cite{anon_htica}]\label{lem:equivariance}
Let $X$ be a random vector on $\RR^\dim$.
Let $A: \RR^\dim \to \RR^\dim$ be an invertible linear transformation.
Then $\Gamma (AX) = A (\Gamma X)$.
\end{lemma}
\fi
%\fi
\iflong
\begin{lemma}\label{lem:innerball}
Let $S = (S_1, \dots, S_n) \in \RR^n$ be an absolutely symmetrically distributed random vector such that
% $\e S = 0$\lnote{superfluous?}
$\e (\abs{S_i}) = 1$ and $\e (\abs{S_i}^{1+\gamma}) \leq M < \infty$ for all $i$. 
Let $S^{(i)}, i=1, \dotsc, N$ be a sample of iid. copies of $S$. Let $Y$ be a random vector, uniformly distributed  in $S^{(1)}, \dotsc, S^{(N)}$. 
Then $ (1-\eps') B_{1}^{\dim} \subseteq \Gamma Y$ whenever
\[
N \geq \left(\frac{16 M \dim^4}{(\eps')^2} \delta'\right)^{\frac{1}{2} + \frac{3}{\gamma}}.
\]
\end{lemma}
\fi
%\begin{proofidea}
%From Lemma \ref{lem:centroid-scaling} we know $\pm e_i \in \Gamma S$. 
%It is enough to apply Lemma \ref{lem:centroid_approximation} to $\pm e_i$. 
%This gives, for any $\theta \in S^{\dim-1}$,  $h_{\Gamma Y} (\theta) \geq h_{\Gamma S} (\theta) -\eps \geq h_{B_1^\dim} (\theta) -\eps \geq (1-\sqrt{\dim} \eps) h_{B_1^\dim}(\theta)$. In particular, $\Gamma Y \supseteq (1-\sqrt{\dim}\eps) B_1^\dim$.
%\end{proofidea}
\begin{proof}
From Lemma \ref{lem:centroid-scaling} we know $\pm e_i \in \Gamma S$. 
It is enough to apply Lemma \ref{lem:centroid_approximation} to $\pm e_i$ with $\eps = \eps'/\sqrt{\dim}$ and $\delta = \delta'/(2\dim)$.
This gives, for any $\theta \in S^{\dim-1}$,  $h_{\Gamma Y} (\theta) \geq h_{\Gamma S} (\theta) -\eps \geq h_{B_1^\dim} (\theta) -\eps \geq (1-\sqrt{\dim} \eps) h_{B_1^\dim}(\theta) = (1-\eps')h_{B_1^\dim}(\theta)$. 
In particular, $\Gamma Y \supseteq (1-\eps') B_1^\dim$.
\end{proof} 

\begin{proposition}[Dual characterization of centroid body]\label{prop:dualcharacterization}
%Let $X$ be a $\dim$-dimensional centrally symmetric random vector with finite first moment xxx. Then 
%\[
%\Gamma X = \{ \e Y \suchthat \text{$Y$ is a random vector such that } (\forall \text{ Borel }T \subseteq \RR^\dim) \measure_Y(T) \leq 2 \measure_X(T)\}.
%\]
Let $X$ be a $\dim$-dimensional random vector with finite first moment, that is, for all $u \in \RR^\dim$ we have $\e (\abs{\inner{u}{X}}) < \infty$. Then 
\iflong
\begin{equation}\label{equ:dualcentroid}
    \Gamma X = \{ \e \bigl(\lambda(X) X \bigr) \suchthat \text{$\lambda:\RR^n \to [-1,1]$ is measurable}\}.
\end{equation}
\else
    $\Gamma X = \{ \e \bigl(\lambda(X) X \bigr) \suchthat \text{$\lambda:\RR^n \to [-1,1]$ is measurable}\}$.
\fi
\end{proposition}
\begin{proof}
Let $K$ denote the rhs of the conclusion.% \eqref{equ:dualcentroid}. 
We will show that $K$ is a non-empty, closed convex set and show that $h_K = h_{\Gamma X}$, which implies \eqref{equ:dualcentroid}.

By definition, $K$ is a non-empty bounded convex set. To see that it is closed, let $(y_k)_k$ be a sequence in $K$ such that $y_k \to y \in \RR^\dim$. 
Let $\lambda_k$ be the function associated to $y_k \in K$  according to the definition of $K$.
Let $\measure_X$ be the distribution of $X$.
We have $\norm{\lambda_k}_{L^\infty(\measure_X)} \leq 1$ and, passing to a subsequence $k_j$, $(\lambda_{k_j})$ converges to $\lambda \in L^\infty(\measure_X)$ in the weak-$*$ topology $\sigma(L^\infty(\measure_X), L^1(\measure_X))$, where $-1 \leq \lambda \leq 1$.
\footnote{This is a standard argument, see \cite{MR2759829} for the background. Map $x \mapsto x_i$ is in $L^1(\measure_X)$. \cite[Theorem 4.13]{MR2759829} gives that $L^1(\measure_X)$ is a separable Banach space. \cite[Theorem 3.16]{MR2759829} (Banach-Alaoglu-Bourbaki) gives that the unit ball in $L^\infty(\measure_X)$ is compact in the weak-* topology. \cite[Theorem 3.28]{MR2759829} gives that the unit ball in $L^\infty(\measure_X)$ is metrizable and therefore sequentially compact in the weak-* topology. Therefore, any bounded sequence in $L^\infty(\measure_X)$ has a convergent subsequence in the weak-* topology.}
This implies $\lim_{j} \e (\lambda_{k_j} (X) X_i) = \lim_j \int_{\RR^\dim} \lambda_{k_j} (x) x_i \ud \measure_X(x) = \int_{\RR^\dim} \lambda(x) x_i \ud \measure_X(x) = \e (\lambda (X) X_i) $.
Thus, we have $y = \lim_j y_{k_j} = \lim_j \e ((\lambda_{k_j}(X) X) = \e (\lambda(X) X)$ and $K$ is closed.

To conclude, we compute $h_K$ and see that it is the same as the definition of $h_{\Gamma X}$. In the following equations $\lambda$ ranges over functions such that $\lambda:\RR^n \to \RR$ is Borel-measurable and $-1 \leq \lambda \leq 1$.
\begin{align*}
h_K(\theta)
&= \sup_{y \in K} \inner{y}{\theta} \\
&= \sup_{\lambda} \e( \lambda(X) \inner{X}{\theta}) \\
\intertext{and setting $\lambda^*(x) = \sign \inner{x}{\theta}$,}
&= \e( \lambda^*(X) \inner{X}{\theta}) \\
&= \e (\abs{\inner{X}{\theta}}).
\end{align*}
\end{proof}

\begin{lemma}[LP]\label{lemma:centroid-lp}
Let $X$ be a random vector uniformly distributed in $\{x^{(i)}\}_{i=1}^{N} \subseteq \RR^\dim$. Let $q \in \RR^\dim$.
Then: 
\begin{enumerate}
\item $\Gamma X = \frac{1}{N} \sum_{i=1}^N [-x^{(i)}, x^{(i)}]$.

\item 
Point $q~\in~\Gamma X$ iff there is a solution $\lambda~\in~\RR^N$ to the following linear feasibility problem:
\begin{equation}\label{eq:lp}
\iflong
\begin{aligned}
&  \frac{1}{N} \sum_{i=1}^N \lambda_i x^{(i)} = q \\
%& y_i \leq 2 f_X(x_i) \quad \forall i\\
% & \sum_i y_i = 1 \\
%& y_1 + \dots + y_N = 1 \\
& -1 \leq \lambda_i \leq 1 \quad \forall i.
\end{aligned}
\else
\frac{1}{N} \sum_{i=1}^N \lambda_i x^{(i)} = q,
%& y_i \leq 2 f_X(x_i) \quad \forall i\\
% & \sum_i y_i = 1 \\
%& y_1 + \dots + y_N = 1 \\
-1 \leq \lambda_i \leq 1 \quad \forall i.
\fi
\end{equation}
\item 
Let $\lambda^*$ be the optimal value of (always feasible) linear program
\begin{equation}\label{eq:lpminkowski}
\begin{aligned}
\iflong
&\lambda^* = \max \lambda \\
\text{s.t. } & \frac{1}{N} \sum_{i=1}^N \lambda_i x^{(i)} = \lambda q \\
% & \sum_i y_i = 1 \\
%& y_1 + \dots + y_N = 1 \\
& -1 \leq \lambda_i \leq 1 \quad \forall i
\else
\lambda^* = \max \lambda, 
\text{s.t. }  \frac{1}{N} \sum_{i=1}^N \lambda_i x^{(i)} = \lambda q, 
% & \sum_i y_i = 1 \\
%& y_1 + \dots + y_N = 1 \\
 \lambda \in [-1,1]^N
\fi
\end{aligned}
\end{equation}
with $\lambda^* = \infty$ if the linear program is unbounded. Then the Minkowski functional of $\Gamma X$ at $q$ is $1/\lambda^*$.
\end{enumerate}
\end{lemma}
%
%Note that in Lemma~\ref{lemma:centroid-lp}, $z(y) = \sum_{i} x_i P_Y(x_i)$ gives the mean of the sample $\{x_i\}$ over the discrete distribution given by $P_Y(x_i) = y_i$.
%This then enables one to take a finite sample $\{x_i\}$ from a general distribution and estimate membership in its centroid body.
\begin{proof}
\begin{enumerate}
\item
This is proven in \cite{MR0279689}.
It is also a special case of Proposition \ref{prop:dualcharacterization}. 
We include an argument here for completeness. 
Let $K := \frac{1}{N} \sum_{i=1}^N [-x^{(i)}, x^{(i)}]$. 
We compute $h_K$ to see it is the same as $h_{\Gamma X}$ in the definition of $\Gamma X$ (Definition \ref{def:centroid-body2}). 
As $K$ and $\Gamma X$ are non-empty compact convex sets, this implies $K = \Gamma X$.
We have 
\begin{align*}
h_K(y) 
&= \sup_{\lambda_i \in [-1,1]} \frac{1}{N} \sum_{i=1}^N \lambda_i x^{(i)} \cdot y \\
&= \max_{\lambda_i \in \{-1,1\}} \frac{1}{N} \sum_{i=1}^N \lambda_i x^{(i)} \cdot y \\
&= \frac{1}{N} \sum_{i=1}^N \abs{ x^{(i)} \cdot y }\\
&= \e (\abs{X \cdot y}).
\end{align*}
\item This follows immediately from part 1. 
\item This follows from part 1 and the definition of Minkowski functional.\qedhere
\end{enumerate}
\end{proof}
\begin{subroutine}[ht]
\caption{Weak Membership Oracle for $\Gamma X$}\label{sub:centroid-oracle}
\begin{algorithmic}[1]
\Require Query point $q \in \RR^\dim$,
samples from symmetric ICA model $X = AS$,
bounds $s_M \geq \sigma_{\max}(A)$, $s_m \leq \sigma_{\min}(A)$,
closeness parameter $\eps$,
failure probability $\delta$.
\Ensure $(\epsilon, \delta)$-weak membership decision for $q \in \Gamma X$.
\State Let $N = \poly(n, M, 1/s_m, s_M, 1/\eps, 1/\delta)$.
\State Let $(x^{(i)})_{i=1}^N$ be an iid. sample of $X$. 
%Let $f_X$ be the uniform discrete density supported on $(x^{(i)})_{i=1}^N$.
\State Check the feasibility of linear program \eqref{eq:lp}. If feasible, output YES, otherwise output NO.
\end{algorithmic}
\end{subroutine}

\begin{proposition}[Correctness of Subroutine \ref{sub:centroid-oracle}]
Let $X=AS$ be given by an ICA model such that for all $i$ we have $\e (\abs{S_i}^{1+\gamma}) \leq M < \infty$, $S_i$ is symmetrically distributed and normalized so that $\e \abs{S_i} = 1$.
Then, given a query point $q \in \RR^\dim$,  $\eps>0$, $\delta > 0$, $s_M \geq \sigma_{\max}(A)$, and $s_m \leq \sigma_{\min}(A)$, Subroutine~\ref{sub:centroid-oracle} is an $\eps$-weak membership oracle for $q$ and $\Gamma X$ with probability $1-\delta$ using time and sample complexity
\(
\poly(n, M, 1/s_m, s_M, 1/\eps, 1/\delta).
\)\lnote{query time should also depend on query, unless we are talking about arithmetic operations}
% Moreover, $s_m /\sqrt{\dim} B_2^\dim \subseteq \Gamma X \subseteq s_M \sqrt{\dim} B_2^\dim$.
\end{proposition}
\begin{proof}
Let $Y$ be uniformly random in $(x^{(i)})_{i=1}^N$. There are two cases corresponding to the guarantees of the oracle: 
\begin{itemize}
\item Case $q \notin (\Gamma X)_\eps$. 
Then there is a hyperplane separating $q$ from $(\Gamma X)_\eps$.
Let $\{x \in \RR^\dim \suchthat a^T x = b \}$ be the separating hyperplane, parameterized so that $a \in \RR^\dim$, $b \in \RR$, $\norm{a} = 1$, $a^T q > b$ and $a^T x \leq b$ for every $x \in (\Gamma X)_\eps$. 
In this case $h_{(\Gamma X)_\eps}(a) \leq b$ and $h_{\Gamma X}(a) \leq b - \eps$.
At the same time, $h_{\Gamma Y}(a) = \e (\abs{a^T Y}) = (1/N) \sum_{i=1}^N \abs{a^T x^{(i)}}$.

We want to apply Lemma~\ref{lem:1-plus-eps-chebyshev} to $a^T X$ to get that $h_{\Gamma Y}(a) = (1/N) \sum_{i=1}^N \abs{a^T x^{(i)}}$ is within $\eps$ of $h_{\Gamma X}(a) = \e ( \abs{a^T X} )$. 
For this we need a bound on the $(1+\gamma)$-moment of $a^T X$. 
We use the bound from \cite[Equation (10)]{anon_htica}: 
$\e (\abs{a^T X}^{1+\gamma}) \leq M \dim s_M^{1+\gamma}$.
Lemma~\ref{lem:1-plus-eps-chebyshev} implies that for
\begin{align} \label{eqn:N-lower-bound}
N \geq 
\max \left\{ \left(\frac{8 M \dim s_M^{1+\gamma}}{\eps^2 \delta}\right)^{3/\gamma}, \left( \frac{8M \dim s_M^{1+\gamma}}{\eps}\right)^{\frac{1}{2} + \frac{1}{\gamma}} \right\},
%%\geq \left(\frac{8 M \dim \sigma_{\max}(A)^{1+\gamma}}{\eps_1^2 \delta}\right)^{3/\gamma},
\end{align}
we have
\[
P\left(\abs{\sum_{i=1}^N \abs{a^T x^{(i)}} - \e (\abs{a^T X})} > \eps\right) \leq \delta.
\]
In particular, with probability at least $1-\delta$ we have $h_{\Gamma Y}(a) \leq b$, which implies $q \notin \Gamma Y$ and, by Lemma \ref{lemma:centroid-lp}, Subroutine \ref{sub:centroid-oracle} outputs NO.


\item Case $q \in (\Gamma X)_{-\eps}$.
Let $y = q + \eps \hat q = q(1+\frac{\eps}{\norm{q}})$.
Let $\alpha = 1+\frac{\eps}{\norm{q}}$.
Then $y \in \Gamma X$.
Invoke Lemma \ref{lem:centroid_approximation} for iid. sample $(x^{(i)})_{i=1}^N$ of $X$ with $p = y$ and $\eps$ equal to some $\eps_1 > 0$ to be fixed later to conclude $y \in (\Gamma Y)_{\eps_1}$.
That is, there exist $z \in \Gamma Y$ such that 
\begin{equation}\label{equ:z}
\norm{z - y} \leq \eps_1.
\end{equation}
Let $w = z/\alpha$.
Given \eqref{equ:z} and the relationships $y=\alpha q$ and $z=\alpha w$, we have 
\begin{equation}\label{equ:perturbation}
\norm{w-q} \leq \norm{z - y} \leq \eps_1.
\end{equation}
From Lemma \ref{lem:innerball} with $\eps'= 1/2$ and equivariance of the centroid body 
(Lemma \ref{lem:equivariance}) 
we get $\Gamma Y \supseteq \frac{\sigma_{\min}(A) }{2 \sqrt{\dim}} B_2^\dim$. This and convexity of $\Gamma Y$ imply $\conv\{\frac{\sigma_{\min}(A) }{2 \sqrt{\dim}} B_2^\dim \cup \{z\}\} \subseteq \Gamma Y$. In particular, the ball around $w$ of radius
\[
r := \left(1-\frac{1}{\alpha}\right) \frac{\sigma_{\min}(A) }{2 \sqrt{\dim}}
\]
is contained in $\Gamma Y$. 
The choice $\eps_1 = r \geq $ and \eqref{equ:perturbation} imply $q \in \Gamma Y$ and Subroutine \ref{sub:centroid-oracle} outputs YES whenever
\[
N \geq \left( \frac{8 M \dim^2}{r^2 \delta} \right)^{\frac{1}{2} + \frac{1}{\gamma}}.
\]
To conclude, remember that $q \in (\Gamma X)_{-\eps}$. Therefore $\norm{q} + \eps \leq \sqrt{\dim} \sigma_{\max}(A)$ (from Lemma \ref{lem:centroid-scaling} and equivariance of the centroid body, Lemma \ref{lem:equivariance}). This implies
\begin{align*}
r 
&= \frac{\eps}{\norm{q} + \eps} \frac{\sigma_{\min}(A) }{2 \sqrt{\dim}} \\
&\geq  \frac{\eps \sigma_{\min}(A) }{2 \dim \sigma_{\max}(A)}
\end{align*}
\end{itemize}
The claim follows.
\end{proof}
\iflong
\begin{lemma}\label{lem:centroid_approximation}
Let $X$ be a $\dim$-dimensional random vector such that for all coordinates $i$ we have $\e (\abs{X_i}^{1+\gamma}) \leq M < \infty$.
Let $p \in \Gamma X$. 
Let $(X^{(i)})_{i=1}^N$ be an iid. sample of $X$.
Let $Y$ be uniformly random in $(X^{(i)})_{i=1}^N$. Let $\eps>0$, $\delta>0$. If $N \geq \left( \frac{8 M \dim^2}{\eps^2 \delta} \right)^{\frac{1}{2} + \frac{3}{\gamma}}$, then, with probability at least $1-\delta$, $p \in (\Gamma Y)_\eps$.
\end{lemma}
\fi
\begin{proof}
%By Proposition \ref{prop:dualcharacterization}, there exists a probability measure $\nu$ such that $p = \int x \ud \nu(x)$ and, via the Radon-Nikodym theorem, there exists a density $f:\RR^\dim \to \RR$ for $\nu$ with respect to $\pr_X$ satisfying $f(x) \leq 2$ for any $x \in \RR^\dim$.
%%whose Radon-Nikodym derivative satisfies $\ud \nu/\ud \pr_X \leq 2$.
By Proposition \ref{prop:dualcharacterization}, there exists a measurable function $\lambda:\RR^\dim \to \RR$, $-1 \leq \lambda \leq 1$ such that $p = \e (X \lambda(X))$.
Let 
\[
z = \frac{1}{N} \sum_{i=1}^N X^{(i)} \lambda(X^{(i)}).
\]
By Proposition \ref{prop:dualcharacterization}, $z \in \Gamma Y$.

We have $\e_{X^{(i)}} (X^{(i)} \lambda (X^{(i)})) = p$ and, for every coordinate $j$,
\[
\e_{X^{(i)}} (\abs{X^{(i)}_j \lambda (X^{(i)})}^{1+\gamma}) 
\leq \e_{X^{(i)}}(\abs{X^{(i)}_j}^{1+\gamma}) 
\leq  M.
\]
By Lemma \ref{lem:1-plus-eps-chebyshev} and for any fixed coordinate $j$ we have, over the choice of $(X^{(i)})_{i=1}^N$,
\[
\pr( \abs{p_j - z_j} \geq \eps/\sqrt{\dim} ) 
\leq \frac{8 M}{(\eps/\sqrt{\dim})^2 N^{\gamma/3}} 
= \frac{8 M \dim}{\eps^2 N^{\gamma/3}}
\]
whenever $N \geq (8M\sqrt{n}/\eps)^{\frac{1}{2} + \frac{1}{\gamma}}$.
A union bound over $\dim$ choices of $j$ gives:
\[
\pr( \norm{p - z} \geq \eps) 
\leq \frac{8 M \dim^2}{\eps^2 N^{\gamma/3}}.
\]
So  
\(
\pr( \norm{p - z} \geq \eps) \leq \delta
\)
whenever
\[
N \geq \left( \frac{8 M \dim^2}{\eps^2 \delta} \right)^{3/\gamma}
\]
and $N \geq (8M\sqrt{n}/\eps)^{\frac{1}{2} + \frac{1}{\gamma}}$.
The claim follows.
%with probability at least $1-\delta$ there exists $z \in \Gamma Y$ such that $\norm{z-p} \leq \eps/xxx$.
\end{proof}


==> theorems.tex <==
%\newcommand{\optionalbreak}{\\ &}
\newcommand{\optionalbreak}{}
%\newtheorem{theorem}{Theorem}
\declaretheorem[name=Theorem]{theorem}

\newtheorem{lemma}{Lemma}
\newtheorem{conjecture}{Conjecture}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}
\newtheorem{remark}{Remark}

\newtheorem{problem}{Problem}
\newtheorem{question}{Question}


